First Demonstration of a Hybrid Cherenkov and Scintillation Detector in a Proof-of-Principle Axion Search at a Beam Dump

This thesis presents the first demonstration of a hybrid Cherenkov and scintillation optical detector at a beam dump facility for a proof-of-principle search for MeV-scale axion-like particles (ALPs). The work utilizes the Coherent CAPTAIN-Mills (CCM) experiment, a 10-ton liquid argon detector at Los Alamos National Laboratory instrumented with 200 PMTs. Coating 80% of the PMTs with wavelength-shifting material while leaving 20% uncoated enables enhanced Cherenkov sensitivity through wavelength discrimination and 2 ns timing resolution. This work includes detailed modeling of $^{22}$Na calibration data, providing the first comprehensive characterization of scintillation and Cherenkov light production and propagation in such a detector, including systematic uncertainties. Using the same source, it demonstrates the first event-by-event separation of Cherenkov radiation from sub-MeV electrons in a high light-yield scintillation detector. Additionally, this work develops machine learning-based position reconstruction with ~5 cm resolution and energy reconstruction with ~10% resolution at 1 MeV. Four observables exploiting Cherenkov timing, wavelength sensitivity, directionality, pulse shape, and event topology are combined into a likelihood ratio test statistic to suppress steady-state backgrounds for $\leq10$ MeV ALP-induced events. No significant excess is observed. Nevertheless, this improved background rejection excludes new regions of ALP mass-coupling parameter space at the 90% confidence level compared to a previous CCM analysis, despite a smaller exposure. Finally, this thesis explores liquid argon applications to supernova neutrino physics in DUNE and discusses next-generation large-scale hybrid optical detectors. These results demonstrate the potential of hybrid Cherenkov-scintillation detectors for future weakly interacting physics experiments.

==> mitthesis-defaultfonts.tex <==
% From mitthesis package
% Documentation: https://ctan.org/pkg/mitthesis

\ProvidesFile{mitthesis-defaultfonts.tex}[2025/09/23 v1.06 Load Computer/Latin Modern text and math fonts]

%% Default fonts
\ifpdftex
	\ClassNoteNoLine{\ClassName}{Loading Computer Modern text and math fonts (default for pdftex)}
	\RequirePackage[T1]{fontenc} % With T1 encoding, pdftex will silently load the cm-super fontset
%   \RequirePackage[]{babel} % load babel (with desired options) if using a language other than English
	\RequirePackage{bm}
\else
	\ClassNoteNoLine{\ClassName}{Loading Latin Modern text and math fonts (default for unicode engines)}
	%
%   \RequirePackage[]{babel} % load babel (with desired options) if using a language other than English
    \RequirePackage[warnings-off={mathtools-colon,mathtools-overbracket},mathbf=sym]{unicode-math}
    % suppress warnings about lack of integration between mathtools and unicode-math.
    % Unicode-math loads fontspec package, but default fonts are not selected by fontspec in this case.
\fi

